LAM-YOLO: Drones-based Small Object Detection on Lighting-Occlusion Attention Mechanism YOLO

Drone-based target detection presents inherent challenges, such as the high density and overlap of targets in drone-based images, as well as the blurriness of targets under varying lighting conditions, which complicates identification. Traditional methods often struggle to recognize numerous densely packed small targets under complex background. To address these challenges, we propose LAM-YOLO, an object detection model specifically designed for drone-based. First, we introduce a light-occlusion attention mechanism to enhance the visibility of small targets under different lighting conditions. Meanwhile, we incroporate incorporate Involution modules to improve interaction among feature layers. Second, we utilize an improved SIB-IoU as the regression loss function to accelerate model convergence and enhance localization accuracy. Finally, we implement a novel detection strategy that introduces two auxiliary detection heads for identifying smaller-scale targets.Our quantitative results demonstrate that LAM-YOLO outperforms methods such as Faster R-CNN, YOLOv9, and YOLOv10 in terms of mAP@0.5 and mAP@0.5:0.95 on the VisDrone2019 public dataset. Compared to the original YOLOv8, the average precision increases by 7.1\%. Additionally, the proposed SIB-IoU loss function shows improved faster convergence speed during training and improved average precision over the traditional loss function.

==> contents/7-analysis.tex <==
% !TEX root = ../main.tex
% \bibliography{../reference.bib}

\section{Analysis} \label{sec:analysis}

==> contents/9-biography.tex <==
% !TEX root = ../main.tex

% Yimian Dai
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figs/biography/Yimian_Dai}}]{Yimian Dai} received his Ph.D. in signal and information processing from Nanjing University of Aeronautics and Astronautics in 2021. During his doctoral studies, he was a visiting Ph.D. student at the University of Copenhagen from March 2018 to September 2018, and at the University of Arizona from October 2018 to October 2020. He is currently an assistant researcher at Nanjing University of Science and Technology, where his research focuses on remote sensing, computer vision, and deep learning.
\end{IEEEbiography}

% Zihao Xiong
\begin{IEEEbiography}[{
\includegraphics[width=1.45in,height=1.3in,clip,keepaspectratio]{./figs/biography/Zihao_Xiong}}]{Zihao Xiong} is currently pursuing the Bachelor degree of Electronic Information Engineering at the School of Information Science and Engineering, Henan University of Technology. 
He is also a research intern at PCALab in Nanjing University of Science and Technology. His research interests include  infrared small target detection, tracking, and super-resolution.
\end{IEEEbiography}



% Fei Zhou
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figs/biography/Fei_Zhou}}]{Fei Zhou}
  received his M.S. degree in electronic engineering from Xinjiang University in 2017, and received Ph.D. degree from College of Electronic and Information Engineering, Nanjing University of Aeronautics and Astronautics. He is currently a lecturer with College of Information Science and Engineering, Henan University of Technology, Zhengzhou, China. His main research interests are signal processing, target detection and image processing. He has published 10+ papers in journals and conferences, such as TGRS, TAES, WACV, etc.
\end{IEEEbiography}

% Xiang Li
\begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.35in,clip,keepaspectratio]{./figs/biography/Xiang_Li}}]{Xiang Li} is an Associate Professor in College of Computer Science, Nankai University. He received the PhD degree from the Department of Computer Science and Technology, Nanjing University of Science and Technology (NJUST) in 2020. There, he started the postdoctoral career in NJUST as a candidate for the 2020 Postdoctoral Innovative Talent Program. In 2016, he spent 8 months as a research intern in Microsoft Research Asia, supervised by Prof. Tao Qin and Prof. Tie-Yan Liu. He was a visiting scholar at Momenta, mainly focusing on monocular perception algorithm. His recent works are mainly on: neural architecture design, CNN/Transformer, object detection/recognition, unsupervised learning, and knowledge distillation. He has published 20+ papers in top journals and conferences such as TPAMI, CVPR, NeurIPS, etc.
\end{IEEEbiography}

% Jian Yang
\begin{IEEEbiography}[{
  \includegraphics[width=1.45in,height=1.3in,clip,keepaspectratio]{./figs/biography/Jian_Yang}}]{Jian Yang} received the PhD degree from Nanjing University of Science and Technology (NJUST) in 2002, majoring in pattern recognition and intelligence systems. From 2003 to 2007, he was a Postdoctoral Fellow at the University of Zaragoza, Hong Kong Polytechnic University and New Jersey Institute of Technology, respectively. From 2007 to present, he is a professor in the School of Computer Science and Technology of NJUST. Currently, he is also a visiting distinguished professor in the College of Computer Science of Nankai University. He is the author of more than 300 scientific papers in pattern recognition and computer vision. His papers have been cited over 40000 times in the Scholar Google. His research interests include pattern recognition and computer vision. Currently, he is/was an associate editor of Pattern Recognition, Pattern Recognition Letters, IEEE Trans. Neural Networks and Learning Systems, and Neurocomputing. He is a Fellow of IAPR. 
\end{IEEEbiography}










